Is Learning in Games Good for the Learners?

We consider a number of questions related to tradeoffs between reward and regret in repeated gameplay between two agents. To facilitate this, we introduce a notion of $\textit{generalized equilibrium}$ which allows for asymmetric regret constraints, and yields polytopes of feasible values for each agent and pair of regret constraints, where we show that any such equilibrium is reachable by a pair of algorithms which maintain their regret guarantees against arbitrary opponents. As a central example, we highlight the case one agent is no-swap and the other's regret is unconstrained. We show that this captures an extension of $\textit{Stackelberg}$ equilibria with a matching optimal value, and that there exists a wide class of games where a player can significantly increase their utility by deviating from a no-swap-regret algorithm against a no-swap learner (in fact, almost any game without pure Nash equilibria is of this form). Additionally, we make use of generalized equilibria to consider tradeoffs in terms of the opponent's algorithm choice. We give a tight characterization for the maximal reward obtainable against $\textit{some}$ no-regret learner, yet we also show a class of games in which this is bounded away from the value obtainable against the class of common "mean-based" no-regret algorithms. Finally, we consider the question of learning reward-optimal strategies via repeated play with a no-regret agent when the game is initially unknown. Again we show tradeoffs depending on the opponent's learning algorithm: the Stackelberg strategy is learnable in exponential time with any no-regret agent (and in polynomial time with any no-$\textit{adaptive}$-regret agent) for any game where it is learnable via queries, and there are games where it is learnable in polynomial time against any no-swap-regret agent but requires exponential time against a mean-based no-regret agent.

==> prelims.tex <==

\section{Preliminaries (Old)}





%we discuss this further in Section \ref{subsec:no-swap-eq}, and show that there is a sense in which this holds for {\it almost all} games. \js{do we use this property anywhere else than section 3?} \wb{it's used for showing Stackelberg = $\Val(0, I)$}
%unique will assume assume the learner has no weakly dominated strategies, i.e.\ there is some Stackelberg equilibrium $\alpha$ such that $\BR(\alpha) = \{b\}$. \wb{May not actually need this}




%\js{moved this to the end, since it is a little disjoint from the generalized equilibrium stuff} 
%\wb{emphasize that sets of generalized equilibria are polytopes}
%, as the roles of the two players in the game may not be identical. In particular, when considering notions of equilibrium for characterizing the sets of strategy profile distributions which repeated learning converges to, there is no {\it a priori} reason to require both players to use identical learning algorithms. For example, 

% \begin{definition}[Repeated Games]
% Definition of ``meta-game'' where players commit to a learning algorithm $\textup{Rep}(G, T)$
% \end{definition}
% \wb{Do we need a formal statement of this, or fine without?}


%dynamic regret (we probably want a simplified characterization of this for our purposes, there's lots of variants)




